Tensor-based modeling/estimation of static channels in IRS-assisted MIMO systems

This paper proposes a tensor-based parametric modeling and estimation framework in multiple-input multiple-output (MIMO) systems assisted by intelligent reflecting surfaces (IRSs). We present two algorithms that exploit the tensor structure of the received pilot signal to estimate the concatenated channel. The first one is an iterative solution based on the alternating least squares algorithm. In contrast, the second method provides closed-form estimates of the involved parameters using the high order single value decomposition. Our numerical results show that our proposed tensor-based methods provide improved performance compared to competing state-of-the-art channel estimation schemes, thanks to the exploitation of the algebraic tensor structure of the combined channel without additional computational complexity.

==> 1preamble.tex <==
%% Packages %%
\usepackage{algorithm}% http://ctan.org/pkg/algorithm
\usepackage{algpseudocode}% http://ctan.org/pkg/algorithmicx
\usepackage{amstext,amsmath,amssymb,exscale,mathtools,bm,gensymb,cite}
\usepackage{psfrag}
\usepackage[none]{hyphenat}
\usepackage{tabularx}
\usepackage[shortlabels]{enumitem}
\usepackage{xcolor}
\usepackage{caption,subcaption,siunitx}
\usepackage[nolist,nohyperlinks]{acronym}
\usepackage{scalerel}
\usepackage{makecell}
\usepackage{graphicx}
\usepackage{acro}   
\usepackage{hyperref}

% Font size of captions
\usepackage[font=small]{caption}
% Blank space before and after section name
%\usepackage{titlesec}
%\titlespacing*{\section}{10pt}{0.750\baselineskip}{0.50\baselineskip}


==> 2acronyms.tex <==
\begin{acronym}[MPC] % Give the longest label here so that the list is nicely aligned
    
    \acro{6G}{sixth generation} 
    
    \acro{AR}{auto-regressive}

    \acro{ADR}{achievable data rate}
    
    \acro{AoA}{angle of arrival}
    
    \acro{AoD}{angle of departure}

    \acro{AWGN}{additive white Gaussian noise}
    
    \acro{B5G}{beyond fifth generation}

    \acro{BS}{base station}

    \acro{BPSK}{binary phase-shift keying}
    
    \acro{IRS}{intelligent reflecting surface}

    \acro{mmWave}{millimeter Wave}
    
    \acro{MIMO}{multiple input multiple output}

    \acro{CSI}{channel state information}

    \acro{DFT}{discrete Fourier transform}

    \acro{HOSVD}{high order single value decomposition}
    
    \acro{LOS}{line of sight}
    
    \acro{MMSE}{minimum mean squared error}

    \acro{NMSE}{normalized mean square error}

    \acro{NLOS}{non-line of sight}
    
    \acro{SNR}{signal-to-noise ratio}

    \acro{SVD}{singular value decomposition}

    \acro{SE}{spectral efficiency}
    
    \acro{UE}{user equipment}
    
    \acro{ULA}{uniform linear array}

    \acro{URA}{uniform rectangular array}

    % Algorithms

    \acro{ALS}{alternating least squares}
    
    \acro{KF}{Kronecker factorization}
    
    \acro{KRF}{Khatri-Rao factorization}

    \acro{LS}{least squares}    
    
\end{acronym}
